Safety Alignment Backfires: Preventing the Re-emergence of Suppressed Concepts in Fine-tuned Text-to-Image Diffusion Models

Fine-tuning text-to-image diffusion models is widely used for personalization and adaptation for new domains. In this paper, we identify a critical vulnerability of fine-tuning: safety alignment methods designed to filter harmful content (e.g., nudity) can break down during fine-tuning, allowing previously suppressed content to resurface, even when using benign datasets. While this "fine-tuning jailbreaking" issue is known in large language models, it remains largely unexplored in text-to-image diffusion models. Our investigation reveals that standard fine-tuning can inadvertently undo safety measures, causing models to relearn harmful concepts that were previously removed and even exacerbate harmful behaviors. To address this issue, we present a novel but immediate solution called Modular LoRA, which involves training Safety Low-Rank Adaptation (LoRA) modules separately from Fine-Tuning LoRA components and merging them during inference. This method effectively prevents the re-learning of harmful content without compromising the model's performance on new tasks. Our experiments demonstrate that Modular LoRA outperforms traditional fine-tuning methods in maintaining safety alignment, offering a practical approach for enhancing the security of text-to-image diffusion models against potential attacks.

==> preamble/acronym.tex <==
\usepackage[acronym,nowarn,section,nogroupskip,nonumberlist]{glossaries}

\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}

\glsdisablehyper{}
\newcommand{\acaps}[1]{{\scshape #1}}
\newacronym[\glslongpluralkey={Conditional Neural Processes}]{cnp}{\acaps{cnp}}{Conditional Neural Process}

% Continual Learning
\newacronym{cl}{\acaps{cl}}{continual learning}
\newacronym{cf}{\acaps{cf}}{catastrophic forgetting}
\newacronym{ewc}{\acaps{ewc}}{Elastic Weight Consolidation}

% Diffusion
\newacronym{cfg}{\acaps{cfg}}{classifier-free guidance}
\newacronym{dco}{\acaps{dco}}{Direct Consistency Optimization}

% LLM
\newacronym{llm}{\acaps{llm}}{large language model}
\newacronym{lora}{\textsc{l}o\textsc{ra}}{low-rank adaptation}
\newacronym{modlora}{\textsc{m}odular \textsc{l}o\textsc{ra}}{modular low-rank adaptation}

\newacronym{peft}{\textsc{peft}}{parameter-efficient fine-tuning}
\newacronym{dpo}{\textsc{dpo}}{direct preference optimization}
\newacronym{ppo}{\textsc{ppo}}{proximal policy optimization}
\newacronym{rlhf}{\textsc{rlhf}}{reinforcement learning from human feedback}

% SAFETY
\newacronym{esd}{\acaps{esd}}{\acaps{esd}}
\newacronym{sdd}{\acaps{sdd}}{\acaps{sdd}}

% METRIC
\newacronym{kid}{\acaps{kid}}{Kernel Inception Distance}
\newacronym{fid}{\acaps{fid}}{Fr\'echet Inception Distance}



==> table/esd_ranks.tex <==
\begin{table}[t]
\caption{ESD with different ranks.}
\label{tab:esd_ranks}
\centering
\begin{tabular}{@{}lrrrrrr@{}}
Module & Rank & \%\textsc{nsfw}{\tiny $\downarrow$} & \%\textsc{nude}{\tiny $\downarrow$} & CLIP{\tiny $\uparrow$} & FID{\tiny $\downarrow$} & LPIPS{\tiny $\downarrow$} \\
SD v1.4 & -- & 73.58 & 33.36 & 0.2746 & 16.543 & -- \\
\midrule
Full & -- & 9.20 & 1.80 & 0.2674 & 17.968 & 0.1610 \\
\midrule
LoRA &  4 & 3.68 & 0.78 & 0.2609 & 18.599 & 0.1952 \\
LoRA &  8 & 3.90 & 0.74 & 0.2615 & 17.954 & 0.1861 \\
LoRA & 16 & 3.88 & 0.74 & 0.2613 & 18.733 & 0.1899 \\
LoRA & 32 & 4.20 & 0.76 & 0.2625 & 18.633 & 0.1834 \\
LoRA & 64 & 4.00 & 0.64 & 0.2637 & 18.813 & 0.1812 \\
\bottomrule
\end{tabular}
\end{table}

==> table/sdd_ranks.tex <==
\begin{table}[t]
\caption{SDD with different ranks.}
\label{tab:sdd_ranks}
\centering
\begin{tabular}{@{}lrrrrrr@{}}
Module & Rank & \%\textsc{nsfw}{\tiny $\downarrow$} & \%\textsc{nude}{\tiny $\downarrow$} & CLIP{\tiny $\uparrow$} & FID{\tiny $\downarrow$} & LPIPS{\tiny $\downarrow$} \\
SD v1.4 & -- & 73.58 & 33.36 & 0.2746 & 16.543 & -- \\
\midrule
Full & -- & 9.20 & 1.80 & 0.2674 & 17.968 & 0.1610 \\
\midrule
LoRA &  4 & 3.68 & 0.78 & 0.2609 & 18.599 & 0.1952 \\
LoRA &  8 & 3.90 & 0.74 & 0.2615 & 17.954 & 0.1861 \\
LoRA & 16 & 3.88 & 0.74 & 0.2613 & 18.733 & 0.1899 \\
LoRA & 32 & 4.20 & 0.76 & 0.2625 & 18.633 & 0.1834 \\
LoRA & 64 & 4.00 & 0.64 & 0.2637 & 18.813 & 0.1812 \\
\bottomrule
\end{tabular}
\end{table}
